VEnhancer: Generative Space-Time Enhancement for Video Generation

We present VEnhancer, a generative space-time enhancement framework that improves the existing text-to-video results by adding more details in spatial domain and synthetic detailed motion in temporal domain. Given a generated low-quality video, our approach can increase its spatial and temporal resolution simultaneously with arbitrary up-sampling space and time scales through a unified video diffusion model. Furthermore, VEnhancer effectively removes generated spatial artifacts and temporal flickering of generated videos. To achieve this, basing on a pretrained video diffusion model, we train a video ControlNet and inject it to the diffusion model as a condition on low frame-rate and low-resolution videos. To effectively train this video ControlNet, we design space-time data augmentation as well as video-aware conditioning. Benefiting from the above designs, VEnhancer yields to be stable during training and shares an elegant end-to-end training manner. Extensive experiments show that VEnhancer surpasses existing state-of-the-art video super-resolution and space-time super-resolution methods in enhancing AI-generated videos. Moreover, with VEnhancer, exisiting open-source state-of-the-art text-to-video method, VideoCrafter-2, reaches the top one in video generation benchmark -- VBench.

==> tables/vbench_quality.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table}[]
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\hline
\textbf{Models} & \textbf{\makecell{Subject\\Consistency}}    & \textbf{\makecell{Background\\Consistency}} & \textbf{\makecell{Temporal\\Flickering}}    & \textbf{\makecell{Motion\\Smoothness}}      & \textbf{\makecell{Aesthetic\\Quality}}      & \textbf{\makecell{Dynamic\\Degree}}         & \textbf{\makecell{Imaging\\Quality}}        & \textbf{\makecell{Object\\Class}}           \\ \hline
Show-1          & 95.53\%                         & 98.02\%                         & \cellcolor[HTML]{F2F2F2}99.12\% & \cellcolor[HTML]{F2F2F2}98.24\% & 57.35\%                         & \cellcolor[HTML]{F2F2F2}44.44\% & 58.66\%                         & \cellcolor[HTML]{F2F2F2}93.07\% \\
LaVie           & 91.41\%                         & 97.47\%                         & 98.30\%                         & 96.38\%                         & 54.94\%                         & \cellcolor[HTML]{F2F2F2}49.72\% & 61.90\%                         & 91.82\%                         \\
Open-Sora       & 92.09\%                         & 97.39\%                         & 98.41\%                         & 95.61\%                         & 57.76\%                         & \cellcolor[HTML]{F2F2F2}48.61\% & 61.51\%                         & 74.98\%                         \\
VideoCrafter-2  & \cellcolor[HTML]{F2F2F2}96.85\% & \cellcolor[HTML]{F2F2F2}98.22\% & 98.41\%                         & 97.73\%                         & 63.13\%                         & 42.50\%                         & \cellcolor[HTML]{F2F2F2}67.22\% & \cellcolor[HTML]{F2F2F2}92.55\% \\
Pika            & 96.76\%                         & \cellcolor[HTML]{F2F2F2}98.95\% & \cellcolor[HTML]{F2F2F2}99.77\% & \cellcolor[HTML]{F2F2F2}99.51\% & \cellcolor[HTML]{F2F2F2}63.15\% & 37.22\%                         & 62.33\%                         & 87.45\%                         \\
Gen-2           & \cellcolor[HTML]{F2F2F2}97.61\% & 97.61\%                         & \cellcolor[HTML]{F2F2F2}99.56\% & \cellcolor[HTML]{F2F2F2}99.58\% & \cellcolor[HTML]{F2F2F2}66.96\% & 18.89\%                         & \cellcolor[HTML]{F2F2F2}67.42\% & 90.92\%                         \\
Ours            & \cellcolor[HTML]{F2F2F2}97.17\% & \cellcolor[HTML]{F2F2F2}98.54\% & 98.46\%                         & 97.75\%                         & \cellcolor[HTML]{F2F2F2}65.89\% & 42.50\%                         & \cellcolor[HTML]{F2F2F2}70.45\% & \cellcolor[HTML]{F2F2F2}93.39\% \\ \hline
\end{tabular}
% \end{table}

==> tables/vbench_semantic.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table}[]
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\hline
\textbf{Models} & \textbf{Multiple Objects}       & \textbf{Human Action}           & \textbf{Color}                  & \textbf{Spatial Relationship}   & \textbf{Scene}                  & \textbf{Appearance Style}       & \textbf{Temporal Style}         & \textbf{Overall Consistency}    \\ \hline
Show-1          & 45.47\%                         & \cellcolor[HTML]{F2F2F2}95.60\% & 86.35\%                         & 53.50\%                         & 47.03\%                         & 23.06\%                         & 25.28\%                         & \cellcolor[HTML]{F2F2F2}27.46\% \\
LaVie           & 33.32\%                         & \cellcolor[HTML]{F2F2F2}96.80\% & 86.39\%                         & 34.09\%                         & \cellcolor[HTML]{F2F2F2}52.69\% & \cellcolor[HTML]{F2F2F2}23.56\% & \cellcolor[HTML]{F2F2F2}25.93\% & 26.41\%                         \\
Open-Sora       & 33.64\%                         & 85.00\%                         & 78.15\%                         & 43.95\%                         & 37.33\%                         & 21.58\%                         & \cellcolor[HTML]{F2F2F2}25.46\% & 26.18\%                         \\
VideoCrafter-2  & 40.66\%                         & \cellcolor[HTML]{F2F2F2}95.00\% & \cellcolor[HTML]{F2F2F2}92.92\% & 35.86\%                         & \cellcolor[HTML]{F2F2F2}55.29\% & \cellcolor[HTML]{F2F2F2}25.13\% & \cellcolor[HTML]{F2F2F2}25.84\% & \cellcolor[HTML]{F2F2F2}28.23\% \\
Pika            & \cellcolor[HTML]{F2F2F2}46.69\% & 88.00\%                         & 85.31\%                         & \cellcolor[HTML]{F2F2F2}65.65\% & 44.80\%                         & 21.89\%                         & 24.44\%                         & 25.47\%                         \\
Gen-2           & \cellcolor[HTML]{F2F2F2}55.47\% & 89.20\%                         & \cellcolor[HTML]{F2F2F2}89.49\% & \cellcolor[HTML]{F2F2F2}66.91\% & 48.91\%                         & 19.34\%                         & 24.12\%                         & 26.17\%                         \\
Ours            & \cellcolor[HTML]{F2F2F2}49.83\% & \cellcolor[HTML]{F2F2F2}95.00\% & \cellcolor[HTML]{F2F2F2}94.41\% & \cellcolor[HTML]{F2F2F2}64.88\% & \cellcolor[HTML]{F2F2F2}51.82\% & \cellcolor[HTML]{F2F2F2}24.32\% & 25.17\%                         & \cellcolor[HTML]{F2F2F2}27.57\% \\ \hline
\end{tabular}
% \end{table}
